Latte-Mix: Measuring Sentence Semantic Similarity with Latent Categorical Mixtures

Measuring sentence semantic similarity using pre-trained language models such as BERT generally yields unsatisfactory zero-shot performance, and one main reason is ineffective token aggregation methods such as mean pooling. In this paper, we demonstrate under a Bayesian framework that distance between primitive statistics such as the mean of word embeddings are fundamentally flawed for capturing sentence-level semantic similarity. To remedy this issue, we propose to learn a categorical variational autoencoder (VAE) based on off-the-shelf pre-trained language models. We theoretically prove that measuring the distance between the latent categorical mixtures, namely Latte-Mix, can better reflect the true sentence semantic similarity. In addition, our Bayesian framework provides explanations for why models finetuned on labelled sentence pairs have better zero-shot performance. We also empirically demonstrate that these finetuned models could be further improved by Latte-Mix. Our method not only yields the state-of-the-art zero-shot performance on semantic similarity datasets such as STS, but also enjoy the benefits of fast training and having small memory footprints.

==> Makefile <==
engine = "pdflatex -interaction=nonstopmode --shell-escape %O %S"
refs = references.bib
# sources = main.tex $(wildcard **/*.tex)
# sources = main.tex $(shell find -print **/*.tex)
sources = main.tex $(shell find . -type f -name '*.tex')

main.pdf: $(sources)
	@latexmk -pdf -pdflatex=${engine} -output-directory='output' -bibtex $<

watch:
	make; \
	(zathura output/main.pdf &); \
	while true; do \
		inotifywait -e modify -q $(sources); \
		make; \
	done
	# @while inotifywait -e modify $(refs) $(sources); do make; done

spell:
	@hunspell -l -t -d en_US -i utf-8 $(sources) \
		| sort \
		| uniq --ignore-case \
		| grep -vxFf dictionary.txt

clean:
	@latexmk -C
	rm -rf output/*

pack:
	rm ../active-inference.tar || true
	cp output/references.bbl references.bbl
	tar -czvf ../active-inference.tar --exclude .git --exclude .gitignore --exclude *.log --exclude output .

.PHONY: watch spell clean


==> figures/layers/sbert_layers.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=.8\linewidth]{figures/layers/sbert_layers.pdf}

\caption{Evaluation of different embedding layers of the pretrained language model BERT. Spearman correlation between the pairwise sentence cosine similarity and the gold labels on STSbenchmark datasets are reported. }
\label{fig:sbert_layers}
\end{figure}


==> figures/layers/word_embedding.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=.8\linewidth]{figures/layers/sbert_layers_wss.pdf}

\caption{Evaluation of different embedding layers of the pretrained language model BERT. Spearman correlation between the pairwise sentence cosine similarity and the gold labels on STSbenchmark datasets are reported. }
\label{fig:layers_word}
\end{figure}


==> sections/background.tex <==
\section{Background}
\label{sec:background}
\subsection{Word/Sentence Vectors}
\subsection{Pretrained Language Model}
\subsection{VAE}

==> tables/sbert_layers.tex <==
\begin{table}
  \centering
  \begin{tabular}{l@{\hskip .2in}c@{\hskip 0.2in}c@{\hskip 0.2in}c@{\hskip 0.2in}c@{\hskip 0.2in}c@{\hskip 0.2in}c@{\hskip 0.2in}c}
\toprule
    Methods &STS15 &SICK-R &STSb \\\midrule
    SBert-Base-1   &69.26 &62.00 &57.36 \\
    SBert-Base-2   &68.89 &62.17 &57.58 \\
    SBert-Base-3   &68.03 &62.32 &54.64 \\
    SBert-Base-11   &79.35 &73.98 &77.48 \\
    SBert-Base-12   &79.09 &72.91 &76.98 \\\hline
    VAE-SBert-Base-1   &71.70 &60.81 &61.22 \\
    VAE-SBert-Base-2   &70.25 &60.47 &61.40 \\
    VAE-SBert-Base-3   &69.67 &60.21 &60.59 \\
    VAE-SBert-Base-11   &80.86 &76.02 &78.17 \\
    VAE-SBert-Base-12   &81.47 &74.63 &78.47 \\
    \bottomrule
  \end{tabular}
  \caption{Evaluation of different embedding layers of Sentence-BERT. Spearman correlation between the pairwise sentence cosine similarity and the gold labels on STSbenchmark datasets are reported. }
  \label{tbl:sbert_layers}
\end{table}

==> tables/senteval_all.tex <==
\begin{table*}
  \centering
  \begin{tabular}{l@{\hskip .2in}c@{\hskip 0.2in}c@{\hskip 0.2in}c@{\hskip 0.2in}c@{\hskip 0.2in}c@{\hskip 0.2in}c@{\hskip 0.2in}c@{\hskip 0.2in}c@{\hskip 0.2in}}
\toprule
    Methods &MR &CR &SUBJ &MPQA &TREC &MRPC &SST2 &SST5 \\\midrule
    Bert-Base  & 81.5 &86.73 &95.22 &88.02 &90.6 &73.68 &85.94 &46.74 \\
    RoBerta-Base  &83.93 &88.24 &95.19 &86.58 &93.2 &74.2 &89.46 &51.27\\
    Bert-Large & & & & & & &  \\
    RoBerta-Large & & & & & & &  \\ \hline
    VAE-Bert-Base  &80.59 &86.6 &95.25 &87.49 &91.4 &73.51 &84.4 &45.97 \\
    VAE-RoBerta-Base &82.17 &84.64 &95.21 &85.87 &89.8 &75.36 &87.1 &46.24  \\
    VAE-Bert-Large &  & & & & & &  \\
    VAE-RoBerta-Large &  & & & & & &  \\ \bottomrule
    SBert-Base  &82.7  &89.04 &94.08 &89.71 &85.2 &75.07 &88.36 &47.38 \\
    SRoBerta-Base &85.17  &90.94 &92.54 &88.77 &88.6 &78.09 &90.55 &52.76  \\
    SBert-Large &  & & & & & &  \\
    SRoBerta-Large &  & & & & & &  \\ \hline
    VAE-SBert-Base  & 81.12 &87.95 &92.97 &89.59 &79.6 &73.57 &84.13 &46.29 \\
    VAE-SRoBerta-Base &84.43  &90.12 &92.26 &88.0 &79.2 &71.83 &91.32 &51.49  \\
    VAE-SBert-Large &  & & & & & &  \\
    VAE-SRoBerta-Large &  & & & & & &  \\ \bottomrule
  \end{tabular}
  \caption{Evaluation of sentence embeddings using the SentEval toolkit. SentEval evaluates sentence embeddings on different sentence classification tasks by training a logistic regression classifier using the sentence embeddings as features. Scores are based on a 10-fold cross-validation.}
  \label{tbl:senteval_all}
\end{table*}

==> tables/senteval_base.tex <==
\begin{table}
  \centering
  \begin{tabular}{l@{\hskip .2in}c@{\hskip 0.2in}c@{\hskip 0.2in}c@{\hskip 0.2in}c@{\hskip 0.2in}c@{\hskip 0.2in}c@{\hskip 0.2in}c@{\hskip 0.2in}c@{\hskip 0.2in}}
\toprule
    Methods &MR &CR &MPQA \\\midrule
    Bert-Base  & 81.50 &86.73 &\textbf{88.02} \\
    Bert-Large &\textbf{84.64} &\textbf{88.77} &86.65 \\
    VAE-Bert-Base  &80.59 &86.60  &87.49 \\
    VAE-Bert-Large &84.19 &88.69 &86.35  \\\hline
    SBert-Base  &82.70  &89.04  &89.71  \\
    SBert-Large &\textbf{84.65}*  &\textbf{91.00}* &\textbf{90.34}* \\
    VAE-SBert-Base  & 81.12 &87.95  &89.59 \\
    VAE-SBert-Large &83.70  &89.85  &90.33   \\\bottomrule
  \end{tabular}
  \caption{Evaluation of sentence embeddings using the SentEval toolkit. SentEval evaluates sentence embeddings on different sentence classification tasks by training a logistic regression classifier using the sentence embeddings as features. Scores are based on a 10-fold cross-validation.}
  \label{tbl:senteval_base}
\end{table}
